Glyph-Based Multiscale Visualization of Turbulent Multi-Physics Statistics

Many scientific and engineering problems involving multi-physics span a wide range of scales. Understanding the interactions across these scales is essential for fully comprehending such complex problems. However, visualizing multivariate, multiscale data within an integrated view where correlations across space, scales, and fields are easily perceived remains challenging. To address this, we introduce a novel local spatial statistical visualization of flow fields across multiple fields and turbulence scales. Our method leverages the curvelet transform for scale decomposition of fields of interest, a level-set-restricted centroidal Voronoi tessellation to partition the spatial domain into local regions for statistical aggregation, and a set of glyph designs that combines information across scales and fields into a single, or reduced set of perceivable visual representations. Each glyph represents data aggregated within a Voronoi region and is positioned at the Voronoi site for direct visualization in a 3D view centered around flow features of interest. We implement and integrate our method into an interactive visualization system where the glyph-based technique operates in tandem with linked 3D spatial views and 2D statistical views, supporting a holistic analysis. We demonstrate with case studies visualizing turbulent combustion data--multi-scalar compressible flows--and turbulent incompressible channel flow data. This new capability enables scientists to better understand the interactions between multiple fields and length scales in turbulent flows.

==> sections/00-Abstract.tex <==
\begin{abstract}
Many scientific and engineering problems involving multi-physics span a wide range of scales. Understanding the interactions across these scales is essential for fully comprehending such complex problems. However, visualizing multivariate, multiscale data within an integrated view where correlations across space, scales, and fields are easily perceived remains challenging. To address this, we introduce a novel local spatial statistical visualization of flow fields across multiple fields and turbulence scales. Our method leverages the curvelet transform for scale decomposition of fields of interest, a level-set-restricted centroidal Voronoi tessellation to partition the spatial domain into local regions for statistical aggregation, and a set of glyph designs that combines information across scales and fields into a single, or reduced set of perceivable visual representations. Each glyph represents data aggregated within a Voronoi region and is positioned at the Voronoi site for direct visualization in a 3D view centered around flow features of interest. We implement and integrate our method into an interactive visualization system where the glyph-based technique operates in tandem with linked 3D spatial views and 2D statistical views, supporting a holistic analysis. We demonstrate with case studies visualizing turbulent combustion data—multi-scalar compressible flows—and turbulent incompressible channel flow data. This new capability enables scientists to better understand the interactions between multiple fields and length scales in turbulent flows.

   %The ABSTRACT is to be in fully-justified italicized text, 
   %between two horizontal lines,
   %in one-column format, 
   %below the author and affiliation %information. 
   %Use the word ``Abstract'' as the title, in 9-point Times, boldface type, 
   %left-aligned to the text, initially capitalized. 
   %The abstract is to be in 9-point, single-spaced type.
   %The abstract may be up to 3 inches (7.62 cm) long. \\
   %Leave one blank line after the abstract, 
   %then add the subject categories according to the ACM Classification Index
%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see https://www.acm.org/publications/computing-classification-system/1998)
% \begin{classification} % according to https://www.acm.org/publications/computing-classification-system/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
   %(see https://www.acm.org/publications/class-2012)
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10003120.10003145.10003147.10010364</concept_id>
       <concept_desc>Human-centered computing~Scientific visualization</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}
\ccsdesc[500]{Human-centered computing~Scientific visualization}



\printccsdesc   
\end{abstract}  


==> sections/01-Introduction.tex <==
\section{Introduction} 
\label{sec:intro}

Understanding turbulent flow physics is crucial in many scientific and engineering problems. For example, turbulence modulates reactions and transport in determining the efficiency and emissions from utilizing sustainable fuels, like hydrogen and ammonia, in engines for power and transportation. Geophysical turbulent flow affects the layout of turbines in wind farms to effectively harness wind energy. Turbulent transport and reactions behind shocks generated in high-speed flows determine the effectiveness of various flame holding strategies in hypersonic flight. Despite the governing equations of turbulent flow being well-known, the inherent multi-scale and nonlinear characteristics of turbulence coupled with multi-physics (e.g., chemical reactions, atomization, radiation) pose significant challenges to fundamental understanding and its control. While advances in high-performance computing have enabled the creation of rich datasets through direct numerical simulations (DNSs), providing accurate statistics to develop new models, the chaotic states and superposed structures at different length scales make studying instantaneous structures difficult. For instance, wall-bounded turbulence involves a wide spectrum of length scales whose importance varies with distance from the wall. In high-speed flows, the separation of these scales widens, affecting phenomena like wall shear stress and energy exchange between velocity components. Consequently, the superposition of these scales complicates understanding energy exchange mechanisms within coherent structures of turbulent flows. 
This complexity further increases when turbulent flows are coupled with multi-physics phenomena. In turbulent reacting flows, for example, the interplay between extraordinarily thin flames and turbulence across decades of length and time scales is central to developing more efficient and cleaner combustion systems. This complexity is heightened in hydrogen-containing, fuel-lean mixtures due to thermo-diffusive instabilities, where flames form intrinsic cellular patterns at small diffusive-reaction scales with length scales modulated by turbulence spanning a broad range of scales from the size of a combustor down to viscous scales where kinetic energy is dissipated. The intrinsic flame instability results in higher burning rates through preferential enrichment of the highly mobile hydrogen fuel depending upon the local flame topology. In turn, the gas expansion from the higher burning rate results in small-scale production of kinetic energy which nonlinearly interacts with kinetic energy generated by large-scale mean velocity gradients through the turbulence cascade and is eventually dissipated. Therefore, advanced analysis and visualization tools are needed to unravel these intricate multi-scale, multi-physics interactions.

From this, we identify two key steps. The first is to separate information by relevant scale and then correlate the emergent spectral characteristics with the spatial features of structures. The second is to visualize the multiscale multiphysics information obtained from the first. For the first step, there exist numerous Fourier-based methods for scale decomposition, including band-pass filtering with discrete Fourier transform and discrete wavelet transform. Of these, we utilize the discrete curvelet transform (CTF)~\cite{doi:10.1137/05064182X} for its preservation of geometric structures across scales, and its ability to relate global spectral information by scale to the local spatial orientation and position of corresponding signal sources via curvelets. It is also important that the scale decomposition preserves spectral energy. Parseval's theorem guarantees this property for %the DFT, orthogonal wavelets, and% 
the CTF stemming from its tight frame property. Thus, the CTF's properties make it well-suited for multiscale geometric analysis, as seen in the works of Bermejo et al.~\cite{BERMEJO-MORENO_PULLIN_2008, BUMANN2022105665}. %The second step is to visualize the multiscale multiphysics information obtained from the first.% 

The CTF scale decomposition yields additional data per scale and field, whose size matches that of the original data. Visualization is therefore made challenging by the large size and quantity of incoming data, which introduces additional storage demands and perceptual demands stemming from the sheer amount of information to be visually processed at once.
Thus, it is crucial that this information be visualized comprehensively and coherently. Spatial statistical aggregation is one effective approach for visualizing large multivariate volumetric data as it organizes it %the data
into smaller regions of aggregate statistics. In prior work on flow visualization, local statistics are computed based on topological features of interest~\cite{bremer2009topological}, then aggregated about volumetric flow features~\cite{9904439}. We advance this direction by applying the level set restricted centroidal Voronoi tessellation (LSRCVT)~\cite{9904439} to multivariate multiscale data, then extending the visualization to visually correlate these statistics with their spatial location in a 3D view. Using the level set restricted centroidal Voronoi tessellation (LSRCVT)~\cite{9904439}, data across all fields and scales is spatially segmented and organized such that it aligns with the flow features from a select field. In combustion analysis, we organize the statistics and glyphs around the flame surface defined by temperature $T$ in kelvin (K). In channel flow analysis, they are organized around coherent structures defined by turbulent kinetic energy $\epsilon_K$. 
With this segmentation, we aggregate the spectral energy derived from the scale decomposition by scale, field, and region (see Section~\ref{sec:aggregation}). This reduces the size of data needed to represent the multiscale multivariate information by several orders of magnitude, making its management and visualization more feasible. 

From here, the remaining challenge comes in visualizing the local multivariate-multiscale statistics. One approach might be to directly encode information across the aggregate region or surface with color seen in other similar approaches~\cite{ccd78f3da756466eb378417b08e49996, 7042344, :10.2312/VisSym/EuroVis07/011-018}. However, color alone may prove insufficient as it can only encode one field at a time. Additional color blending and intensity could be used to encode more information but this may obfuscate the multiscale information. Instead, we might consider using symbols alongside color to encode more information. This prompts the use of glyphs as they can 
%be used to display 
present a lot of information in a singular visual representation. Since glyphs are commonly used to symbolize information at a particular point or region in space, they are a good fit for visualizing aggregate data across a spatial surface. Once the glyphs are placed accordingly, they can either be interpreted individually up close or as a collection from afar. Adding dynamic interaction to these glyphs enhances exploration as users can control the visual representation of information for 
%based on 
the desired level of detail.
%desired. 
For this reason, we design glyphs to encode the LSRCVT-aggregated information by scales, fields, and spatial regions. 
%Compared to the raw multiscale decomposition data, the aggregated data used to render the glyph-based visualization is several orders of magnitudes smaller. %~\ref{sec:evaluation}
%Thus, the data can be visualized locally on a desktop system, without having to rely on cluster computing or out-of-core algorithms. 

% 
%Our contributions are as follows. 
Overall, we present a novel application of symbolic glyphs which combine scales and fields into a reduced set of visual representations. They are applied within a 3D spatial statistical context to summarize multiscale multivariate information along the surface of a volume. This constitutes a novel multiscale visualization which enables direct comparison of multiple fields and scales with the underlying surface geometry. \color{changed} By linking scale dependence to the local surface topology of flow structures, experts can gain valuable insight on how they behave across scales within a multiphysical space. \color{black} Our approach %also 
extends the LSRCVT-based spatial statistical aggregation method, which did not previously allow for direct visualization of the statistics in a 3D spatial context. This aggregation also enables a data reduction strategy that makes multiscale visualization more feasible across larger datasets.

\vspace{-0.15in}








